Signal Propagation in Transformers: Theoretical Perspectives and the Role of Rank Collapse

Transformers have achieved remarkable success in several domains, ranging from natural language processing to computer vision. Nevertheless, it has been recently shown that stacking self-attention layers - the distinctive architectural component of Transformers - can result in rank collapse of the tokens' representations at initialization. The question of if and how rank collapse affects training is still largely unanswered, and its investigation is necessary for a more comprehensive understanding of this architecture. In this work, we shed new light on the causes and the effects of this phenomenon. First, we show that rank collapse of the tokens' representations hinders training by causing the gradients of the queries and keys to vanish at initialization. Furthermore, we provide a thorough description of the origin of rank collapse and discuss how to prevent it via an appropriate depth-dependent scaling of the residual branches. Finally, our analysis unveils that specific architectural hyperparameters affect the gradients of queries and values differently, leading to disproportionate gradient norms. This suggests an explanation for the widespread use of adaptive methods for Transformers' optimization.

==> old.tex <==
\section{Related work}
- works on initialization of transformers
- works on the need of warmup with adam and other on adaptive learning rates
- works on training stabilization
- works on enhancing/replacing the softmax\\

\luca{preliminar: just a commented list of papers}
\cite{wang2022deepnet} introduces DeepNorm, a simple initialization scheme that enables training of transformer models with more than 1000 layers. The initialization is based on rescaling of the residual connections and on the introduction of a gain parameter for the weights of the feed-forward connections and the value projections. In all the evaluations though the authors still use warmup as well as layer normalization, Adam and gradient clipping.

\cite{bachlechner2021rezero} introduces ReZero a simple trick consisting in the addition of a trainable parameter (initialized to zero) to the residual term in residual connection. The authors show that transformers equipped with this simple scheme can be quickly trained without LayerNorm, even for very large depths.

\cite{xiong2020layer} shows that using layer normalization inside the residual connection (Pre-LN) allows training of Transformers without warm-up. However, they claim that SGD cannot achieve performance on par with Adam. Furthermore, parallel works show that Pre-LN can result in sub-optimal performance on neural machine translation tasks. 

\cite{pmlr-v119-huang20f} shows that the need for warm-up comes from the instability in the Adam optimizer combined with gradient vanishing through layer normalization. A new initialization is then introduced that keeps the models update bounded and enables training without warm-up and layer normalization. However, the Adam optimizer is kept and SGD is deemed as sub-optimal for Transformer training.


\cite{liu2020understanding} found that gradient vanishing is not the only issue preventing stable training in transformers. The find that with Pre-LN, vanishing gradient is removed but the resulting performance is sub-optimal as opposed to the cases where Post-LN converges. Interestingly they notice that gradients of all attention modules are unbalanced and they conclude that the only way to optimize Transformer is via adaptive optimizers. Ultimately, they determine that the dependency on residual branches is one of the main factor determining convergence and performance and they introduce a new initialization based on residual rescaling to successfully cope with it.


\cite{zhang2020adaptive} finds that adaptive optimizers are better suited than plain SGD when attention-based models are considered. This is due to the heavy-tailed nature of noise in stochastic gradients found in BERT optimization. The authors find the \emph{adaptive} gradient clipping is effective in reducing the heavy-tail effect and in closing the gap between SGD and Adam.


\cite{liuadam} provides a theoretical justification for the need for warm-up scheduling when adaptive methods are used. In particular, they show that the convergence issue is due to the undesirably large variance of the adaptive learning rate in the early stage of model training. They thus introduce RAdam, which explicitly rectifies the variance and compares favourably with warm-up.


\cite{shleifer2021normformer} introduces NormFormer, a new model that adds three normalization operations to each layer: a Layer Norm after self attention, head-wise scaling of self-attention outputs, and a Layer Norm after the first fully connected layer. The extra operations incur negligible compute cost (+0.4\% parameter increase), but improve pretraining perplexity and downstream
task performance for both causal and masked language models. 


\cite{wang2019learning} modifies the residual connection by introducing multiple links with all previous layers to access lower-level representations in a deep stack. This simple trick allows to train deeper models on several translation tasks.

\cite{nguyen2019transformers} combines three different types of normalization to cope with training instability in transformer models. PRENORM + FIXNORM + SCALENORM significantly improves NMT on low-resource pairs, with the latter two performing comparably in the high-resource setting, but faster.

\cite{dufter2020increasing} Use of learnable temperature for the attention weights. They use it for all queries, values and keys and per dimension. They report the temperature has no effect (empirical study).





\paragraph{Training Instability in Attention-Based Models.}
Successful optimization in Transformers is notoriously hard and requires several tailored training tricks and architectural design choices. Among these, Layer Normalization is, arguably, one of the most important -- and debated -- ones.
In the original architecture \citep{vaswani2017attention}, Layer Normalization was used in the Post-Norm setting, that is, it was placed between the residual blocks in order to stabilize the forward pass by reducing the variance of the inputs to the following sublayer. Later works \citep{chen2018best} found that its inclusion is highly beneficial for the stabilization of the training process. Nevertheless, successful training of Transformers in the Post-Norm setting remains hard without resorting to adaptive methods opportunely combined with strongly hyperparameter-sensitive preliminary warm-up stages \cite{liuadam,zhang2020adaptive,huang2020improving}. Moreover, training instability in this setting is further exacerbated when the optimization of deeper models is required. These considerations have recently led to the introduction of the so-called Pre-Norm variant \cite{wang2019learning,nguyen2010estimating,xiong2020layer}, where layer normalization is used inside the residual connection. \cite{xiong2020layer} show that since Post-LN induces larger gradients in deeper layers than Pre-Norn, networks equipped with the latter can be trained with larger learning rates and without the need of warm-up. Furthermore, Pre-Norm has been found \cite{wang2019learning,nguyen2010estimating,xiong2020layer} to enable training of deeper models without incurring in training instabilities. However, despite making training easier, the use of Pre-LN can lead to inferior performance than its Post-LN counterpart \cite{liu2020understanding, nguyen2019transformers}. This observation has motivated research on replacing or complementing layer norm with carefully designed initialization schemes \cite{zhang2019fixup,liu2020understanding} or additional architectural modifications \cite{bachlechner2021rezero,wang2022deepnet}. In our work we build upon the above research efforts with the goal of shedding new light on the forward and backward passes of attention-based architectures. In particular, we present, for the first time, a rigorous theoretical analysis of signal propagation in Transformer-based neural networks. In doing so, we provide new insights on the role of Layer Normalization, both in the Post-LN and Pre-LN configurations, and of adaptive optimizers. In relation to this, as also observed by \citep{liu2020understanding}, we identify in the different scales of the norms of queries and values gradients one of the possible causes for the necessity of adaptive methods in Transformers optimization and, differently from \citep{liu2020understanding}, we demonstrate that the introduction of a temperature parameter inside the softmax can help SGD in closing the performance gap with Adam. 
\paragraph{Rank Collapse in Attention-Based Models.}
A parallel line of research \citep{dong2021attention} has recently identified an additional key inductive bias characterizing purely attention-based architectures: their input representations lose rank doubly exponentially with depth. The authors identify residual connections as the most effective component to mitigate this phenomenon. However, \citep{dong2021attention} leave the question on the relation between the emergence of rank collapse and optimization unaddressed. Thanks to our analysis of the backward pass, we are able to demonstrate that rank collapse in Transformer architectures leads to vanishingly small gradients of queries and keys, thereby preventing effective training and completing the analysis started by \citep{dong2021attention}.

